Stop&Hop: Early Classification of Irregular Time Series

Early classification algorithms help users react faster to their machine learning model's predictions. Early warning systems in hospitals, for example, let clinicians improve their patients' outcomes by accurately predicting infections. While early classification systems are advancing rapidly, a major gap remains: existing systems do not consider irregular time series, which have uneven and often-long gaps between their observations. Such series are notoriously pervasive in impactful domains like healthcare. We bridge this gap and study early classification of irregular time series, a new setting for early classifiers that opens doors to more real-world problems. Our solution, Stop&Hop, uses a continuous-time recurrent network to model ongoing irregular time series in real time, while an irregularity-aware halting policy, trained with reinforcement learning, predicts when to stop and classify the streaming series. By taking real-valued step sizes, the halting policy flexibly decides exactly when to stop ongoing series in real time. This way, Stop&Hop seamlessly integrates information contained in the timing of observations, a new and vital source for early classification in this setting, with the time series values to provide early classifications for irregular time series. Using four synthetic and three real-world datasets, we demonstrate that Stop&Hop consistently makes earlier and more-accurate predictions than state-of-the-art alternatives adapted to this new problem. Our code is publicly available at https://github.com/thartvigsen/StopAndHop.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the 
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
    \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See Section \label{sec:data}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{These data are not personally identifiable}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate} 
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> figures/prob_def_ists.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/problem_definition.pdf}
    \caption{Early Classification of Irregularly-Sampled Time Series. Vertical dashed lines indicate the time at which a prediction is generated. An ideal early classifiers accurately labels a given time series as early as possible.}
    \label{fig:prob_def}
\end{figure}

==> tables/es_results.tex <==
\begin{table*}[t]
\centering
\caption{Performance (mean (std)) of early multi-label classification on the \texttt{ExtraSensory} dataset. ``$\downarrow$'' indicates ``the smaller the
better'' and ``$\uparrow$'' indicates ``the larger the better''.} \label{tab:seizures}
\vspace{-10pt}
\begin{tabular}{crccccc}
\toprule

\multirow{2.5}{*}{\shortstack[l]{{\scriptsize Time-Steps}\\{\scriptsize Observed}}}  &\multirow{2.5}{*}{\shortstack[r]{{\textbf{Evaluation}}\\{\textbf{Metrics}}}}& \multicolumn{5}{c}{\textbf{Methods}}\\
\cmidrule{3-7}
   &   &LSTM-BD~\cite{ma2016learning} 
                                &E-LSTM~\cite{dennis2018multiple} 
                                &LSTM-CC~\cite{wang2016cnn} 
                                &EARLIEST~\cite{hartvigsen2019adaptive} 
                                &RHC (ours) \\
\midrule
% --- 20% ---
\multirow{7}{*}{20\%}

&Instance-AUC$^\uparrow$     & 0.71 (0.00) & 0.71 (0.00) &          0.74 (0.02) & 0.71 (0.00) & \textbf{0.78} (0.00)\\
&Micro-AUC$^\uparrow$        & 0.70 (0.00) & 0.69 (0.00) & \textbf{0.72} (0.02) & 0.71 (0.00) &          0.68 (0.00)\\
&Macro-AUC$^\uparrow$        & 0.60 (0.00) & 0.62 (0.00) &          0.63 (0.01) & 0.63 (0.01) & \textbf{0.68} (0.00)\\
\cmidrule{2-7}
&Hamming Loss$^\downarrow$   & 0.31 (0.00) & 0.32 (0.00) &          0.31 (0.01) & 0.31 (0.00) & \textbf{0.27} (0.00)\\
&Micro-F1$^\uparrow$         & 0.58 (0.00) & 0.55 (0.00) &          0.58 (0.02) & 0.58 (0.00) & \textbf{0.61} (0.00)\\
&Macro-F1$^\uparrow$         & 0.48 (0.00) & 0.47 (0.00) &          0.46 (0.01) & 0.47 (0.01) &          0.46 (0.00)\\
\midrule
% --- 40% ---
\multirow{7}{*}{40\%}
&Instance-AUC$^\uparrow$     &  0.74 (0.00) & 0.73 (0.00) & 0.77 (0.01) & 0.74 (0.00) & \textbf{0.79} (0.00)\\
&Micro-AUC$^\uparrow$        &  0.73 (0.00) & 0.71 (0.00) & 0.75 (0.01) & 0.74 (0.00) & \textbf{0.78} (0.00)\\
&Macro-AUC$^\uparrow$        &  0.66 (0.00) & 0.64 (0.00) & 0.68 (0.01) & 0.67 (0.00) & \textbf{0.70} (0.00)\\
\cmidrule{2-7}
&Hamming Loss$^\downarrow$   &  0.32 (0.00) & 0.32 (0.00) & 0.29 (0.01) &           0.27 (0.00) & \textbf{0.26} (0.00)\\
&Micro-F1$^\uparrow$         &  0.56 (0.00) & 0.59 (0.00) & 0.60 (0.00) &           0.60 (0.00) & \textbf{0.62} (0.00)\\
&Macro-F1$^\uparrow$         &  0.47 (0.00) & 0.52 (0.00) & 0.48 (0.02) & \textbf{0.53} (0.01) & 0.48 (0.00)\\
\midrule
% --- 60% ---
\multirow{7}{*}{60\%}
&Instance-AUC$^\uparrow$     &  0.76 (0.00) & 0.75 (0.01) & 0.78 (0.01) & 0.77 (0.01) &  \textbf{0.79} (0.00)\\
&Micro-AUC$^\uparrow$        &  0.76 (0.00) & 0.73 (0.01) & 0.77 (0.01) & 0.76 (0.01) &  \textbf{0.78} (0.00)\\
&Macro-AUC$^\uparrow$        &  0.71 (0.00) & 0.67 (0.01) & 0.70 (0.01) & 0.69 (0.01) &           0.70 (0.00)\\
\cmidrule{2-7}
&Hamming Loss$^\downarrow$   &  0.28 (0.00) & 0.32 (0.01) & 0.28 (0.01) &          0.28 (0.00) & \textbf{0.26} (0.00)\\
&Micro-F1$^\uparrow$         &  0.61 (0.00) & 0.63 (0.01) & 0.62 (0.01) & \textbf{0.62} (0.01) & \textbf{0.62} (0.00)\\
&Macro-F1$^\uparrow$         &  0.53 (0.00) & 0.56 (0.01) & 0.53 (0.01) & \textbf{0.55} (0.00) &          0.47 (0.00)\\
\bottomrule
\end{tabular}\label{tab:extrasensory}
\end{table*}


==> tables/es_results_20.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccccccccccc}
% \toprule
% & \multicolumn{9}{c}{\textbf{Metric}}\\
% \cline{2-10}
% \textbf{Method} & Rank. Loss & P-Mac & P-Mic & F1-Mic & AUC-Mic & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% % \textbf{Method} & Ranking Loss ($\downarrow$) & P-Mac ($\uparrow$) & P-Mic ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% \midrule
% % --- preset methods ---
% RNN-BR \cite{ma2016learning} & 3.07 (0.0) & 0.48 (0.0) & 0.57 (0.0) & 0.58 (0.0) & 0.7 (0.0) & 0.71 (0.0) & 0.6 (0.0) & 0.56 (0.0) & 0.48 (0.0) \\
% E-LSTM \cite{dennis2018multiple} & 1.42 (0.03) & 0.7 (0.04) & 0.68 (0.05) & 0.77 (0.03) & 0.94 (0.01) & 0.93 (0.01) & 0.94 (0.01) & 0.83 (0.02) & 0.84 (0.02) \\
% OF-CC \cite{chen2018order} & 3.06 (0.01) & 0.48 (0.02) & 0.58 (0.02) & 0.58 (0.02) & 0.72 (0.02) & 0.74 (0.02) & 0.63 (0.01) & 0.61 (0.02) & 0.51 (0.01) \\
% EARLIEST \cite{hartvigsen2019adaptive} & 3.04 (0.0) & 0.5 (0.0) & 0.59 (0.0) & 0.58 (0.0) & 0.71 (0.0) & 0.71 (0.0) & 0.63 (0.0) & 0.57 (0.0) & 0.5 (0.0) \\
% RHC (ours) & \textbf{3.02 (0.0)} & \textbf{0.54 (0.0)} & \textbf{0.66 (0.01)} & \textbf{0.61 (0.0)} & \textbf{0.77 (0.0)} & \textbf{0.78 (0.0)} & \textbf{0.68 (0.0)} & \textbf{0.67 (0.01)} & \textbf{0.55 (0.01)} \\
% \bottomrule
% \end{tabular}
% \caption{\texttt{ExtraSensory} task with 20\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
% \label{tab:seizures}
% \vspace{-10pt}
% \end{table*}

\begin{table*}[t]
\centering
\caption{Performance (mean (std)) of early multi-label classification  on Human Activity Recognition (\texttt{HAR}) task. ``$\downarrow$'' indicates ``the smaller the
better'' and ``$\uparrow$'' indicates ``the larger the better''.} \label{tab:seizures}
\vspace{-10pt}
\begin{tabular}{llccccc}
\toprule
{\scriptsize Time-Steps}  &\textbf{Evaluation}& \multicolumn{5}{c}{\textbf{Methods}}\\
\cline{3-7}
{\scriptsize Observed}     &\textbf{Metrics}   &RNN-BR~\cite{ma2016learning} 
                                &E-LSTM~\cite{dennis2018multiple} 
                                &OF-CC~\cite{chen2018order} 
                                &EARLIEST~\cite{hartvigsen2019adaptive} 
                                &RHC [ours] \\
\midrule
% --- 20% ---
\multirow{8}{*}{20\%}
&Ranking Loss$^\downarrow$   & 3.07 (0.0) & 1.42 (0.03) & 3.06 (0.01) & 3.04 (0.00) & \textbf{3.02} (0.00)\\
&Micro-Precision$^\uparrow$  & 0.57 (0.0) & 0.68 (0.05) & 0.58 (0.02) & 0.59 (0.00) & \textbf{0.66} (0.01)\\
&Macro-Precision$^\uparrow$  & 0.48 (0.0) & 0.70 (0.04) & 0.48 (0.02) & 0.50 (0.00) & \textbf{0.54} (0.00)\\
&Micro-F1$^\uparrow$         & 0.58 (0.0) & 0.77 (0.03) & 0.58 (0.02) & 0.58 (0.00) & \textbf{0.61} (0.00)\\
&Micro-AUC$^\uparrow$        & 0.70 (0.0) & 0.94 (0.01) & 0.72 (0.02) & 0.71 (0.00) & \textbf{0.68} (0.00)\\
&Instance-AUC$^\uparrow$     & 0.71 (0.0) & 0.93 (0.01) & 0.74 (0.02) & 0.71 (0.00) & \textbf{0.78} (0.00)\\
&Average Precision$^\uparrow$& \\
\midrule
% --- 40% ---
\multirow{8}{*}{40\%}
&Ranking Loss$^\downarrow$   &  3.07 (0.0) & 1.42 (0.03) & 3.01 (0.01) & 3.01 (0.0) & \textbf{3.00} (0.00)\\
&Micro-Precision$^\uparrow$  &  0.57 (0.0) & 0.68 (0.05) & 0.61 (0.02) & 0.61 (0.0) & \textbf{0.67} (0.00)\\
&Macro-Precision$^\uparrow$  &  0.49 (0.0) & 0.70 (0.04) & 0.51 (0.00) & 0.53 (0.0) & \textbf{0.55} (0.00)\\
&Micro-F1$^\uparrow$         &  0.56 (0.0) & 0.77 (0.03) & 0.60 (0.00) & 0.60 (0.0) & \textbf{0.62} (0.00)\\
&Micro-AUC$^\uparrow$        &  0.73 (0.0) & 0.94 (0.01) & 0.75 (0.01) & 0.74 (0.0) & \textbf{0.78} (0.00)\\
&Macro-AUC$^\uparrow$        &  0.66 (0.0) & 0.94 (0.01) & 0.68 (0.01) & 0.67 (0.0) & \textbf{0.70} (0.00)\\
&Instance-AUC$^\uparrow$     &  0.74 (0.0) & 0.93 (0.01) & 0.77 (0.01) & 0.74 (0.0) & \textbf{0.79} (0.00)\\
&Average Precision$^\uparrow$& \\
\midrule
% --- 60% ---
\multirow{8}{*}{60\%}
&Ranking Loss$^\downarrow$   &  3.01 (0.00) & 1.42 (0.03) & 3.00 (0.01) & \textbf{2.96} (0.01) &           3.00 (0.00)\\
&Micro-Precision$^\uparrow$  &  0.64 (0.00) & 0.68 (0.05) & 0.62 (0.02) &          0.64 (0.00) &  \textbf{0.66} (0.00)\\
&Macro-Precision$^\uparrow$  &  0.57 (0.00) & 0.70 (0.04) & 0.55 (0.02) & \textbf{0.57} (0.00) &  \textbf{0.56} (0.00)\\
&Micro-F1$^\uparrow$         &  0.61 (0.00) & 0.77 (0.03) & 0.62 (0.01) &          0.62 (0.01) &           0.62 (0.00)\\
&Micro-AUC$^\uparrow$        &  0.76 (0.00) & 0.94 (0.01) & 0.77 (0.01) &          0.76 (0.01) &  \textbf{0.78} (0.00)\\
&Macro-AUC$^\uparrow$        &  0.71 (0.00) & 0.94 (0.01) & 0.70 (0.01) &          0.69 (0.01) &           0.70 (0.00)\\
&Instance-AUC$^\uparrow$     &  0.76 (0.00) & 0.93 (0.01) & 0.78 (0.01) &          0.77 (0.01) &  \textbf{0.79} (0.00)\\
&Average Precision$^\uparrow$& \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/es_results_40.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{9}{c}{\textbf{Metric}}\\
\cline{2-10}
\textbf{Method} & Rank. Loss & P-Mac & P-Mic & F1-Mic & AUC-Mic & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% \textbf{Method} & Ranking Loss ($\downarrow$) & P-Mac ($\uparrow$) & P-Mic ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
\midrule
% --- preset methods ---
RNN-BR \cite{ma2016learning} & 3.07 (0.0) & 0.49 (0.0) & 0.57 (0.0) & 0.56 (0.0) & 0.73 (0.0) & 0.74 (0.0) & 0.66 (0.0) & 0.6 (0.0) & 0.53 (0.0) \\
% E-LSTM \cite{dennis2018multiple} & 1.42 (0.03) & 0.7 (0.04) & 0.68 (0.05) & 0.77 (0.03) & 0.94 (0.01) & 0.93 (0.01) & 0.94 (0.01) & 0.83 (0.02) & 0.84 (0.02) \\
OF-CC \cite{chen2018order} & 3.01 (0.01) & 0.51 (0.0) & 0.61 (0.02) & 0.6 (0.0) & 0.75 (0.01) & 0.77 (0.01) & 0.68 (0.01) & 0.63 (0.02) & 0.53 (0.02) \\
EARLIEST \cite{hartvigsen2019adaptive} & 3.01 (0.0) & 0.53 (0.0) & 0.61 (0.0) & 0.6 (0.0) & 0.74 (0.0) & 0.74 (0.0) & 0.67 (0.0) & 0.61 (0.0) & 0.54 (0.0) \\
RHC (ours) & \textbf{3.0 (0.0)} & \textbf{0.55 (0.0)} & \textbf{0.67 (0.0)} & \textbf{0.62 (0.0)} & \textbf{0.78 (0.0)} & \textbf{0.79 (0.0)} & \textbf{0.7 (0.0)} & \textbf{0.68 (0.0)} & \textbf{0.57 (0.0) }\\
\bottomrule
\end{tabular}
\caption{\texttt{ExtraSensory} task with 40\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
\label{tab:seizures}
\vspace{-10pt}
\end{table*}

==> tables/es_results_60.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{9}{c}{\textbf{Metric}}\\
\cline{2-10}
\textbf{Method} & Rank. Loss & P-Mac & P-Mic & F1-Mic & AUC-Mic & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% \textbf{Method} & Ranking Loss ($\downarrow$) & P-Mac ($\uparrow$) & P-Mic ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
\midrule
% --- preset methods ---
RNN-BR \cite{ma2016learning} & 3.01 (0.0) & 0.57 (0.0) & 0.64 (0.0) & 0.61 (0.0) & 0.76 (0.0) & 0.76 (0.0) & 0.71 (0.0) & 0.66 (0.0) & 0.58 (0.01) \\
% E-LSTM \cite{dennis2018multiple} & 1.42 (0.03) & 0.7 (0.04) & 0.68 (0.05) & 0.77 (0.03) & 0.94 (0.01) & 0.93 (0.01) & 0.94 (0.01) & 0.83 (0.02) & 0.84 (0.02) \\
OF-CC \cite{chen2018order} & 3.0 (0.01) & 0.55 (0.02) & 0.62 (0.02) & 0.62 (0.01) & 0.77 (0.01) & 0.78 (0.01) & 0.7 (0.01) & 0.67 (0.02) & 0.57 (0.02) \\
EARLIEST \cite{hartvigsen2019adaptive} & \textbf{2.96 (0.01)} & \textbf{0.57 (0.0)} & 0.64 (0.0) & 0.62 (0.01) & 0.76 (0.01) & 0.77 (0.01) & 0.69 (0.01) & 0.66 (0.0) & \textbf{0.6 (0.0)} \\
RHC (ours) & 3.0 (0.0) & \textbf{0.56 (0.0)} & \textbf{0.66 (0.0)} & 0.62 (0.0) & \textbf{0.78 (0.0)} & \textbf{0.79 (0.0)} & 0.7 (0.0) & \textbf{0.68 (0.0)} & 0.57 (0.0) \\
\bottomrule
\end{tabular}
\caption{\texttt{ExtraSensory} task with 60\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
\label{tab:seizures}
\vspace{-10pt}
\end{table*}

==> tables/har_results.tex <==
\begin{table*}[t]
\centering
\caption{Performance (mean (std)) of early multi-label classification on the Human Activity Recognition (\texttt{HAR}) dataset. ``$\downarrow$'' indicates ``the smaller the
better'' and ``$\uparrow$'' indicates ``the larger the better''.} \label{tab:seizures}
\vspace{-10pt}
\begin{tabular}{crcccccc}
\toprule
% {\scriptsize Time-Steps}  &\textbf{Evaluation}& \multicolumn{5}{c}{\textbf{Methods}}\\
\multirow{2.5}{*}{\shortstack[l]{{\scriptsize Time-Steps}\\{\scriptsize Observed}}}  &\multirow{2.5}{*}{\shortstack[r]{{\textbf{Evaluation}}\\{\textbf{Metrics}}}} & \multicolumn{6}{c}{\textbf{Methods}}\\
\cmidrule{3-8}
% {\scriptsize Observed}     &\textbf{Metrics}   &LSTM-BD~\cite{ma2016learning} 
&                               &LSTM-BD~\cite{ma2016learning} 
                                &E-LSTM~\cite{dennis2018multiple} 
                                &LSTM-CC~\cite{wang2016cnn} 
                                &EARLIEST~\cite{hartvigsen2019adaptive} 
                                &RHC \cite{hartvigsen2020recurrent} 
                                &MO-RL (ours)\\
\midrule
% --- 20% ---
\multirow{7}{*}{20\%}
&Instance-AUC$^\uparrow$     & 0.88 (0.00) & 0.85 (0.00) & 0.90 (0.02) & \textbf{0.92} (0.00) & 0.90 (0.01)          & -\\
&Micro-AUC$^\uparrow$        & 0.86 (0.00) & 0.85 (0.00) & 0.88 (0.01) & 0.91 (0.00)          & \textbf{0.92} (0.00) & -\\
&Macro-AUC$^\uparrow$        & 0.86 (0.00) & 0.84 (0.00) & 0.88 (0.02) & 0.91 (0.00)          & \textbf{0.93} (0.00) & -\\
\cmidrule{2-8}
&Hamming Loss$^\downarrow$   & 0.18 (0.00) & 0.21 (0.00) & 0.17 (0.01) & 0.13 (0.00) & \textbf{0.12} (0.01) & -\\
&Micro-F1$^\uparrow$         & 0.62 (0.00) & 0.57 (0.00) & 0.66 (0.03) & 0.74 (0.00) & \textbf{0.76} (0.02) & -\\
&Macro-F1$^\uparrow$         & 0.62 (0.00) & 0.57 (0.00) & 0.65 (0.03) & 0.74 (0.00) & \textbf{0.76} (0.02) & -\\
\midrule
% --- 40% ---
\multirow{7}{*}{40\%}
&Instance-AUC$^\uparrow$     & 0.91 (0.00)   & 0.89 (0.00)   & 0.92 (0.02)   &          0.94 (0.00)   & 0.95 (0.00) & \textbf{0.96} (0.00)\\
&Micro-AUC$^\uparrow$        & 0.90 (0.00)   & 0.90 (0.00)   & 0.92 (0.02)   &          0.92 (0.00)   & 0.95 (0.00) & \textbf{0.96} (0.00) \\
&Macro-AUC$^\uparrow$        & 0.91 (0.00)   & 0.89 (0.00)   & 0.92 (0.02)   &          0.93 (0.00)   & 0.95 (0.00) & \textbf{0.96} (0.00) \\
\cmidrule{2-8}
&Hamming Loss$^\downarrow$   & 0.17 (0.00)   & 0.17 (0.01) & 0.15 (0.01) & 0.10 (0.00) & 0.09 (0.00) & \textbf{0.08} (0.00) \\
&Micro-F1$^\uparrow$         & 0.65 (0.00)   & 0.67 (0.02) & 0.72 (0.02) & 0.79 (0.00) & 0.81 (0.00) & \textbf{0.84} (0.00) \\
&Macro-F1$^\uparrow$         & 0.63 (0.00)   & 0.68 (0.02) & 0.72 (0.02) & 0.79 (0.00) & 0.81 (0.00) & \textbf{0.84} (0.00) \\
\midrule
% --- 60% ---
\multirow{7}{*}{60\%}
&Instance-AUC$^\uparrow$     & 0.92 (0.00)   & 0.93 (0.01)   & 0.93 (0.01)   & 0.94 (0.00)   & 0.96 (0.00) & \textbf{0.97} (0.00) \\
&Micro-AUC$^\uparrow$        & 0.92 (0.00)   & 0.94 (0.01)   & 0.93 (0.01)   & 0.93 (0.00)   & \textbf{0.97} (0.00) & \textbf{0.97} (0.00) \\
&Macro-AUC$^\uparrow$        & 0.90 (0.00)   & 0.94 (0.01)   & 0.93 (0.01)   & 0.94 (0.00)   & \textbf{0.97} (0.00) & \textbf{0.97} (0.00) \\
\cmidrule{2-8}
&Hamming Loss$^\downarrow$   & 0.13 (0.00) & 0.13 (0.02) & 0.13 (0.01) & 0.10 (0.00) & \textbf{0.07} (0.00) & \textbf{0.07} (0.00) \\
&Micro-F1$^\uparrow$         & 0.74 (0.00) & 0.77 (0.03) & 0.75 (0.02) & 0.80 (0.01) & 0.85 (0.00) & \textbf{0.86} (0.00) \\
&Macro-F1$^\uparrow$         & 0.74 (0.00) & 0.78 (0.03) & 0.74 (0.02) & 0.80 (0.01) & 0.85 (0.01) & \textbf{0.86} (0.00) \\
\bottomrule
\end{tabular}\label{tab:har}
\end{table*}


==> tables/har_results_20.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lccccccccccc}
% \toprule
% & \multicolumn{8}{c}{\textbf{Metric}}\\
% \cline{2-9}
% \textbf{Method} & Ranking Loss ($\downarrow$) & Prec-Mac ($\uparrow$) & Prec-Mic ($\uparrow$) & F1-Mac ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac \\
% \midrule
% % --- preset methods ---
% RNN-BR \cite{ma2016learning} & 1.61 (0.0) &  0.65 (0.0) & 0.64 (0.0) & 0.62 (0.0) & 0.62 (0.0) & 0.86 (0.0) & 0.88 (0.0) & 0.86 (0.0)
% \\
% E-LSTM \cite{dennis2018multiple} & 1.64 (0.0) & 0.57 (0.0) & 0.56 (0.0) & 0.57 (0.0) & 0.57 (0.0) & 0.85 (0.0) & 0.85 (0.0) & 0.84 (0.0) \\
% RNN-CC \cite{wang2016cnn} & 1.57 (0.04) & 0.65 (0.02) & 0.63 (0.02) & 0.65 (0.03) & 0.66 (0.03) & 0.88 (0.01) & 0.9 (0.02) & 0.88 (0.02) \\
% EARLIEST \cite{hartbigsen2019adaptibe} & \textbf{1.47 (0.0)} & \textbf{0.75 (0.0)} & \textbf{0.72 (0.0)} & \textbf{0.74 (0.0)} & \textbf{0.74 (0.0)} & \textbf{0.91 (0.0)} & \textbf{0.92 (0.0)} & \textbf{0.91 (0.0)} \\
% RHC (ours) & 1.52 (0.03) & 0.73 (0.02) & 0.73 (0.02) & 0.71 (0.02) & 0.72 (0.02) & \textbf{0.91 (0.00)} & \textbf{0.92 (0.00)} & \textbf{0.91 (0.00)} \\
% \bottomrule
% \end{tabular}
% \caption{\texttt{HAR} task with 20\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
% \label{tab:seizures}
% %\bspace{-10pt}
% \end{table*}


%%---------Old Version---------------------------------------
%\begin{table*}[t]
%\centering
%\caption{\texttt{HAR} task with $20\%$ of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.} \label{tab:seizures}
%\vspace{-10pt}
%{\small
%\begin{tabular}{rcccccccccccc}
%\toprule
%& \multicolumn{9}{c}{\textbf{Metric}}\\
%\cline{2-10}
%\textbf{Method} 
%        & Ranking Loss$^\downarrow$ 
%        & P-Mac$^\uparrow$
%        & P-Mic 
%        & F1-Mic 
%        & AUC-Mic 
%        & AUC-Inst 
%        & AUC-Mac 
%        & AP-Mic & AP-Mac \\
%% \textbf{Method} & Ranking Loss ($\downarrow$) & P-Mac ($\uparrow$) & P-Mic ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
%\midrule
%% --- preset methods ---
%RNN-BR \cite{ma2016learning}          & 1.61 (0.0)        & 0.65 (0.0)        & 0.64 (0.0)         & 0.62 (0.0)        & 0.86 (0.0)        &0.88 (0.0)         & 0.86 (0.0) & 0.66 (0.0) & 0.7 (0.0) \\
%E-LSTM \cite{dennis2018multiple}      & 1.64 (0.0)        & 0.57 (0.0)        & 0.56 (0.0)         & 0.57 (0.0)        & 0.85 (0.0)        &0.85 (0.0)         & 0.84 (0.0) & 0.63 (0.0) & 0.67 (0.0) \\
%OF-CC \cite{chen2018order}            & 1.57 (0.04)       & 0.65 (0.02)       & 0.63 (0.02)        & 0.66 (0.03)       & 0.88 (0.01)       &0.9 (0.02)         & 0.88 (0.02) & 0.69 (0.03) & 0.73 (0.03) \\
%EARLIEST \cite{hartvigsen2019adaptive}&\textbf{1.47 (0.0)}&\textbf{0.75 (0.0)}& 0.72 (0.0)         &\textbf{0.74 (0.0)}&\textbf{0.91 (0.0)}&\textbf{0.92 (0.0)}& \textbf{0.91 (0.0)} & 0.73 (0.0) & 0.79 (0.0) \\
%RHC (ours)                            & 1.52 (0.03)       & 0.73 (0.02)       &\textbf{0.73 (0.02)}& 0.72 (0.02)       &\textbf{0.91 (0.0)}&\textbf{0.92(0.01)}& \textbf{0.91 (0.0)} & \textbf{0.77 (0.02)} & \textbf{0.8 (0.02)} \\
%\bottomrule
%\end{tabular}
%}
%\end{table*}
%%---------------------------------------


\begin{table*}[t]
\centering
\caption{Performance (mean (std)) of early multi-label classification  on Human Activity Recognition (\texttt{HAR}) task. ``$\downarrow$'' indicates ``the smaller the
better'' and ``$\uparrow$'' indicates ``the larger the better''.} \label{tab:seizures}
\vspace{-10pt}
\begin{tabular}{llccccc}
\toprule
{\scriptsize Time-Steps}  &\textbf{Evaluation}& \multicolumn{5}{c}{\textbf{Methods}}\\
\cline{3-7}
{\scriptsize Observed}     &\textbf{Metrics}   &RNN-BR~\cite{ma2016learning} 
                                &E-LSTM~\cite{dennis2018multiple} 
                                &OF-CC~\cite{chen2018order} 
                                &EARLIEST~\cite{hartvigsen2019adaptive} 
                                &RHC [ours] \\
\midrule
% --- 20% ---
\multirow{8}{*}{20\%}
&Ranking Loss$^\downarrow$   & 1.61 (0.00)   &1.64 (0.00)    &1.57 (0.04)    &\textbf{1.47} (0.00)   &         1.52 (0.03)\\
&Micro-Precision$^\uparrow$  & 0.65 (0.00)   &0.57 (0.00)    &0.65 (0.02)    &\textbf{0.75} (0.00)   &         0.73 (0.02)\\
&Macro-Precision$^\uparrow$  & 0.64 (0.00)   &0.56 (0.00)    &0.63 (0.02)    &         0.72 (0.00)   &\textbf{0.73} (0.02)\\
&Micro-F1$^\uparrow$         & 0.62 (0.00)   &0.57 (0.00)    &0.66 (0.03)    &\textbf{0.74} (0.00)   &         0.72 (0.02)\\
&Micro-AUC$^\uparrow$        & 0.86 (0.00)   &0.85 (0.00)    &0.88 (0.01)    &\textbf{0.91} (0.00)   &\textbf{0.91} (0.00)\\
&Macro-AUC$^\uparrow$        & 0.86 (0.00)   &0.84 (0.00)    &0.88 (0.02)    &\textbf{0.91} (0.00)   &\textbf{0.91} (0.00)\\
&Instance-AUC$^\uparrow$     & 0.88 (0.00)   &0.85 (0.00)    &0.90 (0.02)    &\textbf{0.92} (0.00)   &\textbf{0.92} (0.01)\\
&Average Precision$^\uparrow$& \\
\midrule
% --- 40% ---
\multirow{8}{*}{40\%}
&Ranking Loss$^\downarrow$   & 1.59 (0.00)   & 1.53 (0.02)   & 1.50 (0.02)   &          1.44 (0.0)   & \textbf{1.43} (0.00)\\
&Micro-Precision$^\uparrow$  & 0.65 (0.00)   & 0.62 (0.02)   & 0.70 (0.02)   &          0.79 (0.0)   & \textbf{0.81} (0.00)\\
&Macro-Precision$^\uparrow$  & 0.64 (0.00)   & 0.64 (0.02)   & 0.70 (0.03)   &          0.80 (0.0)   & \textbf{0.81} (0.00)\\
&Micro-F1$^\uparrow$         & 0.65 (0.00)   & 0.67 (0.02)   & 0.72 (0.02)   &          0.79 (0.0)   & \textbf{0.81} (0.00)\\
&Micro-AUC$^\uparrow$        & 0.90 (0.00)   & 0.90 (0.00)   & 0.92 (0.02)   &          0.92 (0.0)   & \textbf{0.93} (0.00)\\
&Macro-AUC$^\uparrow$        & 0.91 (0.00)   & 0.89 (0.00)   & 0.92 (0.02)   &          0.93 (0.0)   & \textbf{0.94} (0.00)\\
&Instance-AUC$^\uparrow$     & 0.91 (0.00)   & 0.89 (0.00)   & 0.92 (0.02)   & \textbf{0.94} (0.0)   & \textbf{0.94} (0.00)\\
&Average Precision$^\uparrow$& \\
\midrule
% --- 60% ---
\multirow{8}{*}{60\%}
&Ranking Loss$^\downarrow$   & 1.48 (0.00)   & 1.42 (0.03)   & 1.48 (0.04)   & 1.43 (0.01)   &  \textbf{1.4} (0.01)\\
&Micro-Precision$^\uparrow$  & 0.72 (0.00)   & 0.68 (0.05)   & 0.72 (0.01)   & 0.80 (0.01)   & \textbf{0.82} (0.01)\\
&Macro-Precision$^\uparrow$  & 0.72 (0.00)   & 0.70 (0.04)   & 0.73 (0.01)   & 0.81 (0.00)   & \textbf{0.83} (0.01)\\
&Micro-F1$^\uparrow$         & 0.74 (0.00)   & 0.77 (0.03)   & 0.75 (0.02)   & 0.80 (0.01)   & \textbf{0.83} (0.00)\\
&Micro-AUC$^\uparrow$        & 0.92 (0.00)   & 0.94 (0.01)   & 0.93 (0.01)   & 0.93 (0.00)   & \textbf{0.95} (0.00)\\
&Macro-AUC$^\uparrow$        & 0.90 (0.00)   & 0.94 (0.01)   & 0.93 (0.01)   & 0.94 (0.00)   & \textbf{0.95} (0.00)\\
&Instance-AUC$^\uparrow$     & 0.92 (0.00)   & 0.93 (0.01)   & 0.93 (0.01)   & 0.94 (0.00)   & \textbf{0.95} (0.00)\\
&Average Precision$^\uparrow$& \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/har_results_40.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lccccccccccc}
% \toprule
% & \multicolumn{8}{c}{\textbf{Metric}}\\
% \cline{2-9}
% \textbf{Method} & Ranking Loss ($\downarrow$) & Prec-Mac ($\uparrow$) & Prec-Mic ($\uparrow$) & F1-Mac ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac \\
% \midrule
% % --- preset methods ---
% RNN-BR \cite{ma2016learning} & 1.59 (0.00) & 0.64 (0.00) & 0.65 (0.00) & 0.63 (0.00) & 0.65 (0.00) & 0.9 (0.00) & 0.91 (0.00) & 0.91 (0.00)
% \\
% E-LSTM \cite{dennis2018multiple} & 1.45 (0.03) & 0.66 (0.05) & 0.64 (0.05) & 0.76 (0.03) & 0.75 (0.03) & 0.93 (0.01) & 0.92 (0.02) & 0.93 (0.01) \\
% RNN-CC \cite{wang2016cnn} & 1.5 (0.03) & 0.7 (0.03) & 0.7 (0.03) & 0.72 (0.02) & 0.72 (0.02) & 0.92 (0.02) & 0.92 (0.02) & 0.92 (0.02) \\
% EARLIEST \cite{hartvigsen2019adaptive} & 1.44 (0.0) & 0.8 (0.0) & 0.79 (0.0) & 0.79 (0.0) & 0.79 (0.0) & 0.92 (0.0) & 0.94 (0.0) & 0.93 (0.0) \\
% RHC (ours) & \textbf{1.43 (0.0)} & \textbf{0.81 (0.0)} & \textbf{0.8 (0.0)} & \textbf{0.81 (0.0)} & \textbf{0.81 (0.0)} & \textbf{0.93 (0.0)} & \textbf{0.94 (0.0)} & \textbf{0.94 (0.0)} \\
% \bottomrule
% \end{tabular}
% \caption{\texttt{HAR} task with 40\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
% \label{tab:seizures}
% %\vspace{-10pt}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccccccccccc}
% \toprule
% & \multicolumn{9}{c}{\textbf{Metric}}\\
% \cline{2-10}
% \textbf{Method} & Rank. Loss & P-Mac & P-Mic & F1-Mic & AUC-Mic & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% % \textbf{Method} & Ranking Loss ($\downarrow$) & P-Mac ($\uparrow$) & P-Mic ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% \midrule
% % --- preset methods ---
% RNN-BR \cite{ma2016learning} & 1.59 (0.0) & 0.64 (0.0) & 0.65 (0.0) & 0.65 (0.0) & 0.9 (0.0) & 0.91 (0.0) & 0.91 (0.0) & 0.77 (0.0) & 0.79 (0.0) \\
% E-LSTM \cite{dennis2018multiple} & 1.53 (0.02) & 0.64 (0.02) & 0.62 (0.02) & 0.67 (0.02) & 0.9 (0.0) & 0.89 (0.0) & 0.89 (0.0) & 0.73 (0.01) & 0.76 (0.01) \\
% OF-CC \cite{chen2018order} & 1.5 (0.02) & 0.7 (0.03) & 0.7 (0.02) & 0.72 (0.02) & 0.92 (0.02) & 0.92 (0.02) & 0.92 (0.02) & 0.78 (0.03) & 0.8 (0.02) \\
% EARLIEST \cite{hartvigsen2019adaptive} & 1.44 (0.0) & 0.8 (0.0) & 0.79 (0.0) & 0.79 (0.0) & 0.92 (0.0) & \textbf{0.94 (0.0)} & 0.93 (0.0) & 0.81 (0.0) & 0.83 (0.0) \\
% RHC (ours) & \textbf{1.43 (0.0)} & \textbf{0.81 (0.0)} & \textbf{0.8 (0.0)} & \textbf{0.81 (0.0)} & \textbf{0.93 (0.0)} & \textbf{0.94 (0.0)} & \textbf{0.94 (0.0)} & \textbf{0.83 (0.0)} & \textbf{0.87 (0.0)} \\
% \bottomrule
% \end{tabular}
% \caption{\texttt{HAR} task with 40\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
% \label{tab:seizures}
% \vspace{-10pt}
% \end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{9}{c}{\textbf{Metric}}\\
\cline{2-10}
\textbf{Method} & Rank. Loss & P-Mac & P-Mic & F1-Mic & AUC-Mic & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% \textbf{Method} & Ranking Loss ($\downarrow$) & P-Mac ($\uparrow$) & P-Mic ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
\midrule
% --- preset methods ---
RNN-BR \cite{ma2016learning}  0.77 (0.0) & 0.79 (0.0) \\
E-LSTM \cite{dennis2018multiple}  &  & 0.73 (0.01) & 0.76 (0.01) \\
OF-CC \cite{chen2018order}  & 0.92 (0.02) & 0.78 (0.03) & 0.8 (0.02) \\
EARLIEST \cite{hartvigsen2019adaptive}  0.81 (0.0) & 0.83 (0.0) \\
RHC (ours) \textbf{0.94 (0.0)} & \textbf{0.83 (0.0)} & \textbf{0.87 (0.0)} \\
\bottomrule
\end{tabular}
\caption{\texttt{HAR} task with 40\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
\label{tab:seizures}
\vspace{-10pt}
\end{table*}


==> tables/har_results_60.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lccccccccccc}
% \toprule
% & \multicolumn{8}{c}{\textbf{Metric}}\\
% \cline{2-9}
% \textbf{Method} & Ranking Loss ($\downarrow$) & Prec-Mac ($\uparrow$) & Prec-Mic ($\uparrow$) & F1-Mac ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac \\
% \midrule
% % --- preset methods ---
% RNN-BR \cite{ma2016learning} & 1.46 (0.00) & 0.74 (0.00) & 0.73 (0.00) & 0.75 (0.00) & 0.75 (0.00) & 0.91 (0.00) & 0.93 (0.00) & 0.91 (0.00)\\
% E-LSTM \cite{dennis2018multiple} & 1.45 (0.03) & 0.66 (0.05) & 0.64 (0.05) & 0.76 (0.03) & 0.75 (0.03) & 0.93 (0.01) & 0.92 (0.02) & 0.93 (0.01) \\
% RNN-CC \cite{wang2016cnn} & 1.46 (0.02) & 0.75 (0.02) & 0.75 (0.02) & 0.76 (0.02) & 0.77 (0.02) & 0.93 (0.01) & 0.93 (0.02) & 0.93 (0.02) \\
% EARLIEST \cite{hartvigsen2019adaptive} & 1.41 (0.00) & 0.79 (0.00) & 0.77 (0.00) & 0.78 (0.00) & 0.78 (0.00) & 0.92 (0.00) & 0.94 (0.00) & 0.93 (0.00) \\
% RHC (ours) & \textbf{1.39 (0.00)} & \textbf{0.82 (0.00)} & \textbf{0.81 (0.00)} & \textbf{0.81 (0.00)} &  \textbf{0.81 (0.00)} & \textbf{0.95 (0.00)} & \textbf{0.95 (0.00)} & \textbf{0.95 (0.00)} \\
% \bottomrule
% \end{tabular}
% \caption{\texttt{HAR} task with 60\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
% \label{tab:seizures}
% %\vspace{-10pt}
% \end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{9}{c}{\textbf{Metric}}\\
\cline{2-10}
\textbf{Method} & Rank. Loss & P-Mac & P-Mic & F1-Mic & AUC-Mic & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
% \textbf{Method} & Ranking Loss ($\downarrow$) & P-Mac ($\uparrow$) & P-Mic ($\uparrow$) & F1-Mic ($\uparrow$) & AUC-Mic ($\uparrow$) & AUC-Inst & AUC-Mac & AP-Mic & AP-Mac \\
\midrule
% --- preset methods ---
RNN-BR \cite{ma2016learning} & 1.48 (0.0) & 0.72 (0.0) & 0.72 (0.0) & 0.74 (0.0) & 0.92 (0.0) & 0.92 (0.0) & 0.9 (0.0) & 0.79 (0.0) & 0.81 (0.0) \\
E-LSTM \cite{dennis2018multiple} & 1.42 (0.03) & 0.7 (0.04) & 0.68 (0.05) & 0.77 (0.03) & 0.94 (0.01) & 0.93 (0.01) & 0.94 (0.01) & 0.83 (0.02) & 0.84 (0.02) \\
OF-CC \cite{chen2018order} & 1.48 (0.04) & 0.73 (0.01) & 0.72 (0.01) & 0.75 (0.02) & 0.93 (0.01) & 0.93 (0.01) & 0.93 (0.01) & 0.81 (0.03) & 0.83 (0.02) \\
EARLIEST \cite{hartvigsen2019adaptive} & 1.43 (0.01) & 0.81 (0.0) & 0.8 (0.01) & 0.8 (0.01) & 0.93 (0.0) & 0.94 (0.0) & 0.94 (0.0) & 0.84 (0.01) & 0.86 (0.02) \\
RHC (ours) & \textbf{1.4 (0.01)} & \textbf{0.83 (0.01}) & \textbf{0.82 (0.01}) & \textbf{0.83 (0.0)} & \textbf{0.95 (0.0)} & \textbf{0.95 (0.0)} & \textbf{0.95 (0.0)} & \textbf{0.88 (0.01}) & \textbf{0.9 (0.01)} \\
\bottomrule
\end{tabular}
\caption{\texttt{HAR} task with 60\% of the timesteps. \textit{Mac} indicates \textit{Macro}, \textit{Mic} indicates \textit{Micro}, \textit{Inst} indicates \textit{Instance}.}
\label{tab:seizures}
\vspace{-10pt}
\end{table*}

==> tex/full_bib.tex <==
% --- Datasets ---

@inproceedings{hartvigsen2018early,
  title={Early Prediction of MRSA Infections using Electronic Health Records},
  author={Hartvigsen, Thomas and Sen, Cansu and Brownell, Sarah and Teeple, Erin and Kong, Xiangnan and Rundensteiner, Elke A},
  booktitle={HEALTHINF},
  pages={156--167},
  year={2018}
}

@article{gupta2020early,
  title={An Early Classification Approach for Multivariate Time Series of On-Vehicle Sensors in Transportation},
  author={Gupta, Ashish and Gupta, Hari Prabhat and Biswas, Bhaskar and Dutta, Tanima},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  year={2020},
  publisher={IEEE}
}

@inproceedings{brunskill2013sample,
  title={Sample complexity of multi-task reinforcement learning},
  author={Brunskill, Emma and Li, Lihong},
  booktitle={UAI},
  pages={122--131},
  year={2013}
}

@article{silver2016mastering,
  title={Mastering the game of Go with deep neural networks and tree search},
  author={Silver, David and Huang, Aja and Maddison, Chris J and Guez, Arthur and Sifre, Laurent and Van Den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and others},
  journal={nature},
  volume={529},
  number={7587},
  pages={484},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{mnih2013playing,
  title={Playing atari with deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
  journal={arXiv preprint arXiv:1312.5602},
  year={2013}
}

@article{vaizman2017recognizing,
  title={Recognizing detailed human context in the wild from smartphones and smartwatches},
  author={Vaizman, Yonatan and Ellis, Katherine and Lanckriet, Gert},
  journal={IEEE Pervasive Computing},
  volume={16},
  number={4},
  pages={62--74},
  year={2017},
  publisher={IEEE}
}

@inproceedings{anguita2013public,
  title={A public domain dataset for human activity recognition using smartphones.},
  author={Anguita, Davide and Ghio, Alessandro and Oneto, Luca and Parra, Xavier and Reyes-Ortiz, Jorge Luis},
  booktitle={ESANN},
  year={2013}
}

@article{briggs2012acoustic,
  title={Acoustic classification of multiple simultaneous bird species: A multi-instance multi-label approach},
  author={Briggs, Forrest and Lakshminarayanan, Balaji and Neal, Lawrence and Fern, Xiaoli Z and Raich, Raviv and Hadley, Sarah JK and Hadley, Adam S and Betts, Matthew G},
  journal={The Journal of the Acoustical Society of America},
  volume={131},
  number={6},
  pages={4640--4650},
  year={2012},
  publisher={Acoustical Society of America}
}


% --- Multi-label Learning ---
@inproceedings{nam2019learning,
  title={Learning Context-dependent Label Permutations for Multi-label Classification},
  author={Nam, Jinseok and Kim, Young-Bum and Mencia, Eneldo Loza and Park, Sunghyun and Sarikaya, Ruhi and F{\"u}rnkranz, Johannes},
  booktitle={ICML},
  pages={4733--4742},
  year={2019}
}

@inproceedings{fujita2019end,
  title={End-to-End Neural Speaker Diarization with Permutation-Free Objectives},
  author={Fujita, Yusuke and Kanda, Naoyuki and Horiguchi, Shota and Nagamatsu, Kenji and Watanabe, Shinji},
  booktitle={Interspeech},
  year={2019}
}

@inproceedings{yang2018sgm,
  title={SGM: Sequence Generation Model for Multi-label Classification},
  author={Yang, Pengcheng and Sun, Xu and Li, Wei and Ma, Shuming and Wu, Wei and Wang, Houfeng},
  booktitle={COLING},
  pages={3915--3926},
  year={2018}
}

@inproceedings{vinyals2015order,
  title={Order matters: Sequence to sequence for sets},
  author={Vinyals, Oriol and Bengio, Samy and Kudlur, Manjunath},
  booktitle={ICLR},
  year={2017}
}

@inproceedings{nam2017maximizing,
  title={Maximizing subset accuracy with recurrent neural networks in multi-label classification},
  author={Nam, Jinseok and Menc{\'\i}a, Eneldo Loza and Kim, Hyunwoo J and F{\"u}rnkranz, Johannes},
  booktitle={NeurIPS},
  pages={5413--5423},
  year={2017}
}

@inproceedings{chen2018order,
  title={Order-free RNN with visual attention for multi-label classification},
  author={Chen, Shang-Fu and Chen, Yi-Chen and Yeh, Chih-Kuan and Wang, Yu-Chiang Frank},
  booktitle={AAAI},
  year={2018}
}

@inproceedings{wang2016cnn,
  title={Cnn-rnn: A unified framework for multi-label image classification},
  author={Wang, Jiang and Yang, Yi and Mao, Junhua and Huang, Zhiheng and Huang, Chang and Xu, Wei},
  booktitle={CVPR},
  pages={2285--2294},
  year={2016}
}

@article{yao2017learning,
  title={Learning to diagnose from scratch by exploiting dependencies among labels},
  author={Yao, Li and Poblenz, Eric and Dagunts, Dmitry and Covington, Ben and Bernard, Devon and Lyman, Kevin},
  journal={arXiv preprint arXiv:1710.10501},
  year={2017}
}

@inproceedings{tsai2020order,
  title={Order-free Learning Alleviating Exposure Bias in Multi-label Classification},
  author={Tsai, Che-Ping and Lee, Hung-Yi},
  booktitle={AAAI},
  year={2020}
}


% --- Early Classification ---
@inproceedings{dennis2018multiple,
  title={Multiple instance learning for efficient sequential data classification on resource-constrained devices},
  author={Dennis, Don and Pabbaraju, Chirag and Simhadri, Harsha Vardhan and Jain, Prateek},
  booktitle={NeurIPS},
  pages={10953--10964},
  year={2018}
}

@article{martinez2019adaptive,
  title={Adaptive early classification of temporal sequences using deep reinforcement learning},
  author={Martinez, Coralie and Ramasso, Emmanuel and Perrin, Guillaume and Rombaut, Mich{\`e}le},
  journal={Knowledge-Based Systems},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{wiens2012patient,
  title={Patient risk stratification for hospital-associated c. diff as a time-series classification task},
  author={Wiens, Jenna and Horvitz, Eric and Guttag, John V},
  booktitle={NeurIPS},
  pages={467--475},
  year={2012}
}

@incollection{sutton2000policy,
  title={Policy gradient methods for reinforcement learning with function approximation},
  author={Sutton, Richard S and McAllester, David A and Singh, Satinder P and Mansour, Yishay},
  booktitle={NeurIPS},
  pages={1057--1063},
  year={2000}
}

@incollection{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  booktitle={ICLR},
  year={2014}
}


@incollection{schulman2015gradient,
  title={Gradient estimation using stochastic computation graphs},
  author={Schulman, John and Heess, Nicolas and Weber, Theophane and Abbeel, Pieter},
  booktitle={NeurIPS},
  pages={3528--3536},
  year={2015}
}

@inproceedings{xu2015show,
  title={Show, attend and tell: Neural image caption generation with visual attention},
  author={Xu, Kelvin and Ba, Jimmy and Kiros, Ryan and Cho, Kyunghyun and Courville, Aaron and Salakhudinov, Ruslan and Zemel, Rich and Bengio, Yoshua},
  booktitle={ICML},
  pages={2048--2057},
  year={2015}
}

@misc{graves2013generating,
  title={Generating sequences with recurrent neural networks},
  author={Graves, Alex},
  journal={arXiv preprint arXiv:1308.0850},
  year={arXiv, 2013}
}

@inproceedings{mikolov2010recurrent,
  title={Recurrent neural network based language model},
  author={Mikolov, Tom{\'a}{\v{s}} and Karafi{\'a}t, Martin and Burget, Luk{\'a}{\v{s}} and {\v{C}}ernock{\`y}, Jan and Khudanpur, Sanjeev},
  booktitle={ISCA},
  year={2010}
}

@inproceedings{graves2013speech,
  title={Speech recognition with deep recurrent neural networks},
  author={Graves, Alex and Mohamed, Abdel-rahman and Hinton, Geoffrey},
  booktitle={IEEE ICASSP},
  pages={6645--6649},
  year={2013}
}

@misc{cirecsan2012multi,
  title={Multi-column deep neural networks for image classification},
  author={Cire{\c{s}}an, Dan and Meier, Ueli and Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:1202.2745},
  year={arXiv, 2012}
}

@article{elman1990finding,
  title={Finding structure in time},
  author={Elman, Jeffrey L},
  journal={Cognitive science},
  volume={14},
  number={2},
  pages={179--211},
  year={1990},
  publisher={Wiley Online Library}
}

@article{bengio1994learning,
  title={Learning long-term dependencies with gradient descent is difficult},
  author={Bengio, Yoshua and Simard, Patrice and Frasconi, Paolo},
  journal={IEEE Transactions on Neural Networks},
  volume={5},
  number={2},
  pages={157--166},
  year={1994}
}

@inproceedings{ye2009time,
  title={Time series shapelets: a new primitive for data mining},
  author={Ye, Lexiang and Keogh, Eamonn},
  booktitle={ACM SIGKDD},
  pages={947--956},
  year={2009}
}

@inproceedings{mnih2014recurrent,
  title={Recurrent models of visual attention},
  author={Mnih, Volodymyr and Heess, Nicolas and Graves, Alex and Kavukcuoglu, Koray},
  booktitle={NeurIPS},
  pages={2204--2212},
  year={2014}
}

@article{parrish2013classifying,
  title={Classifying with confidence from incomplete information},
  author={Parrish, Nathan and Anderson, Hyrum S and Gupta, Maya R and Hsiao, Dun Yu},
  journal={Journal of Machine Learning Research},
  volume={14},
  number={1},
  pages={3561--3589},
  year={2013}
}

@inproceedings{lin2015reliable,
  title={Reliable early classification on multivariate time series with numerical and categorical attributes},
  author={Lin, Yu-Feng and Chen, Hsuan-Hsu and Tseng, Vincent S and Pei, Jian},
  booktitle={PAKDD},
  pages={199--211},
  year={2015}
}

@misc{srivastava2015highway,
  title={Highway networks},
  author={Srivastava, Rupesh Kumar and Greff, Klaus and Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:1505.00387},
  year={arXiv, 2015}
}

@article{bengio2015conditional,
  title={Conditional computation in neural networks for faster models},
  author={Bengio, Emmanuel and Bacon, Pierre-Luc and Pineau, Joelle and Precup, Doina},
  journal={arXiv preprint arXiv:1511.06297},
  year={arXiv, 2015}
}


@inproceedings{huang2017length,
  title={Length Adaptive Recurrent Model for Text Classification},
  author={Huang, Zhengjie and Ye, Zi and Li, Shuangyin and Pan, Rong},
  booktitle={CIKM},
  pages={1019--1027},
  year={2017}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural Computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997}
}

@article{he2015early,
  title={Early classification on multivariate time series},
  author={He, Guoliang and Duan, Yong and Peng, Rong and Jing, Xiaoyuan and Qian, Tieyun and Wang, Lingling},
  journal={Neurocomputing},
  volume={149},
  pages={777--787},
  year={2015}
}

@inproceedings{xing2011extracting,
  title={Extracting interpretable features for early classification on time series},
  author={Xing, Zhengzheng and Pei, Jian and Yu, Philip S and Wang, Ke},
  booktitle={SDM},
  pages={247--258},
  year={2011}
}

@article{xing2012early,
  title={Early classification on time series},
  author={Xing, Zhengzheng and Pei, Jian and Yu, Philip S},
  journal={Knowledge and Information Systems},
  volume={31},
  number={1},
  pages={105--127},
  year={2012}
}

@inproceedings{xing2009early,
  title={Early Prediction on Time Series: A Nearest Neighbor Approach},
  author={Xing, Zhengzheng and Pei, Jian and Yu, Phillip},
  booktitle={IJCAI},
  pages={1297--1302},
  year={2009}
}


@article{johnson2016mimic,
  title={MIMIC-III, a freely accessible critical care database},
  author={Johnson, Alistair EW and Pollard, Tom J and Shen, Lu and Lehman, Li-wei H and Feng, Mengling and Ghassemi, Mohammad and Moody, Benjamin and Szolovits, Peter and Celi, Leo Anthony and Mark, Roger G},
  journal={Scientific Data},
  volume={3},
  year={2016}
}

@article{shortreed2011informing,
  title={Informing sequential clinical decision-making through reinforcement learning: an empirical study},
  author={Shortreed, Susan M and Laber, Eric and Lizotte, Daniel J and Stroup, T Scott and Pineau, Joelle and Murphy, Susan A},
  journal={Machine Learning},
  volume={84},
  number={1-2},
  pages={109--136},
  year={2011}
}

@article{williams1992simple,
  title={Simple statistical gradient-following algorithms for connectionist reinforcement learning},
  author={Williams, Ronald J},
  journal={Machine Learning},
  volume={8},
  number={3-4},
  pages={229--256},
  year={1992}
}

@inproceedings{karlsson2016early,
  title={Early Random Shapelet Forest},
  author={Karlsson, Isak and Papapetrou, Panagiotis and Bostr{\"o}m, Henrik},
  booktitle={International Conference on Discovery Science},
  pages={261--276},
  year={2016}
}

@article{ghalwash2012early,
  title={Early classification of multivariate temporal observations by extraction of interpretable shapelets},
  author={Ghalwash, Mohamed F and Obradovic, Zoran},
  journal={BMC Bioinformatics},
  volume={13},
  number={1},
  pages={195},
  year={2012}
}

@inproceedings{guez2008adaptive,
  title={Adaptive Treatment of Epilepsy via Batch-mode Reinforcement Learning.},
  author={Guez, Arthur and Vincent, Robert D and Avoli, Massimo and Pineau, Joelle},
  booktitle={AAAI},
  pages={1671--1678},
  year={2008}
}

@inproceedings{lizotte2010efficient,
  title={Efficient reinforcement learning with multiple reward functions for randomized controlled trial analysis},
  author={Lizotte, Daniel J and Bowling, Michael H and Murphy, Susan A},
  booktitle={ICML},
  pages={695--702},
  year={2010}
}

@techreport{lizotte2009assessing,
  title={Assessing confidence in policies learned from sequential randomized trials},
  author={Lizotte, Daniel J and Laber, Eric and Murphy, Susan A},
  year={2009},
  institution={Technical Report, Department of Statistics, University of Michigan, Ann Arbor, Michigan}
}

@article{pineau2007constructing,
  title={Constructing evidence-based treatment strategies using methods from computer science},
  author={Pineau, Joelle and Bellemare, Marc G and Rush, A John and Ghizaru, Adrian and Murphy, Susan A},
  journal={Drug and Alcohol Dependence},
  volume={88},
  pages={S52--S60},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{li2014early,
  title={Early classification of ongoing observation},
  author={Li, Kang and Li, Sheng and Fu, Yun},
  booktitle={ICDM},
  pages={310--319},
  year={2014}
}

@article{mori2017reliable,
  title={Reliable early classification of time series based on discriminating the classes over time},
  author={Mori, Usue and Mendiburu, Alexander and Keogh, Eamonn and Lozano, Jose A},
  journal={Data Mining and Knowledge Discovery},
  volume={31},
  number={1},
  pages={233--263},
  year={2017}
}

@article{sen2017crest,
title={CREST - Risk Prediction for Clostridium Difficile Infection Using Multimodal Data Mining},
author={Sen, Cansu and Hartvigsen, Thomas and Rundensteiner, Elke and Claypool, Kajal},
journal={Machine Learning and Knowledge Discovery in Databases},
pages = {49-60},
year={2017}}


@inproceedings{ma2016learning,
  title={Learning activity progression in lstms for activity detection and early detection},
  author={Ma, Shugao and Sigal, Leonid and Sclaroff, Stan},
  booktitle={CVPR},
  pages={1942--1950},
  year={2016}
}

@inproceedings{cho2014learning,
  title={Learning phrase representations using RNN encoder-decoder for statistical machine translation},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Gulcehre, Caglar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  booktitle={EMNLP},
  pages={1724--1734},
  year={2014}
}

@inproceedings{weber2014lstm,
  title={Lstm-based early recognition of motion patterns},
  author={Weber, Markus and Liwicki, Marcus and Stricker, Didier and Scholzel, Christopher and Uchida, Seiichi},
  booktitle={ICPR},
  pages={3552--3557},
  year={2014},
  organization={IEEE}
}

@misc{graves2016adaptive,
  title={Adaptive computation time for recurrent neural networks},
  author={Graves, Alex},
  journal={arXiv preprint arXiv:1603.08983},
  year={arXiv, 2016},
}

@misc{bengio2013estimating,
  title={Estimating or propagating gradients through stochastic neurons for conditional computation},
  author={Bengio, Yoshua and L{\'e}onard, Nicholas and Courville, Aaron},
  journal={arXiv preprint arXiv:1308.3432},
  year={arXiv, 2013}
}

@misc{schmidhuber2012self,
  title={Self-delimiting neural networks},
  author={Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:1210.0118},
  year={arXiv, 2012}
}

@inproceedings{keogh2006intelligent,
  title={Intelligent icons: Integrating lite-weight data mining and visualization into GUI operating systems},
  author={Keogh, Eamonn and Wei, Li and Xi, Xiaopeng and Lonardi, Stefano and Shieh, Jin and Sirowy, Scott},
  booktitle={ICDM},
  pages={912--916},
  year={2006}
}

@inproceedings{bridle1990training,
  title={Training stochastic model recognition algorithms as networks can lead to maximum mutual information estimation of parameters},
  author={Bridle, John S},
  booktitle={NeurIPS},
  year={1990}
}

@inproceedings{ghalwash2013extraction,
  title={Extraction of interpretable multivariate patterns for early diagnostics},
  author={Ghalwash, Mohamed F and Radosavljevic, Vladan and Obradovic, Zoran},
  booktitle={ICDM},
  pages={201--210},
  year={2013}
}

@inproceedings{ghalwash2014utilizing,
  title={Utilizing temporal patterns for estimating uncertainty in interpretable early decision making},
  author={Ghalwash, Mohamed F and Radosavljevic, Vladan and Obradovic, Zoran},
  booktitle={SIGKDD},
  pages={402--411},
  year={2014},
}

@article{andrzejak2001indications,
  title={Indications of nonlinear deterministic and finite-dimensional structures in time series of brain electrical activity: Dependence on recording region and brain state},
  author={Andrzejak, Ralph G and Lehnertz, Klaus and Mormann, Florian and Rieke, Christoph and David, Peter and Elger, Christian E},
  journal={Physical Review E},
  volume={64},
  number={6},
  pages={061907},
  year={2001},
  publisher={APS}
}

@inproceedings{kawala2013predictions,
  title={Pr{\'e}dictions d'activit{\'e} dans les r{\'e}seaux sociaux en ligne},
  author={Kawala, Fran{\c{c}}ois and Douzal-Chouakria, Ahlame and Gaussier, Eric and Dimert, Eustache},
  booktitle={4i{\`e}me conf{\'e}rence sur les mod{\`e}les et l'analyse des r{\'e}seaux: Approches math{\'e}matiques et informatiques},
  pages={16},
  year={2013}
}

@article{mori2018early,
  title={Early classification of time series by simultaneously optimizing the accuracy and earliness},
  author={Mori, Usue and Mendiburu, Alexander and Dasgupta, Sanjoy and Lozano, Jose A},
  journal={IEEE transactions on neural networks and learning systems},
  volume={29},
  number={10},
  pages={4569 -- 4578},
  year={2018},
  publisher={IEEE}
}

@inproceedings{coralie2018deep,
  title={A deep reinforcement learning approach for early classification of time series},
  author={Coralie, Martinez and Perrin, Guillaume and Ramasso, E and Rombaut Mich{\`e}lle},
  booktitle={EUSIPCO},
  year={2018}
}

@inproceedings{hartvigsen2019adaptive,
  title={Adaptive-Halting Policy Network for Early Classification},
  author={Hartvigsen, Thomas and Sen, Cansu and Kong, Xiangnan and Rundensteiner, Elke},
  booktitle={SIGKDD},
  pages={101--110},
  year={2019}
}


@article{BLS04,
  title={Learning multi-label scene classification},
  author    = {Matthew R. Boutell and
               Jiebo Luo and
               Xipeng Shen and
               Christopher M. Brown},
  journal={Pattern Recognition},
  volume={37},
  number={9},
  pages={1757 -- 1771},
  year={2004}
}


@article{ZJL20,
  title={Multi-label Prediction in Time Series Data using Deep Neural Networks},
  author    = {Wenyu Zhang and
               Devesh K. Jha and
               Emil Laftchiev and
               Daniel Nikovski},
  title     = {Multi-label Prediction in Time Series Data using Deep Neural Networks},
  journal   = {arXiv preprint},
  volume    = {abs/2001.10098},
  year      = {2020}
}
